MotionDiffuser: Controllable Multi-Agent Motion Prediction using Diffusion

We present MotionDiffuser, a diffusion based representation for the joint distribution of future trajectories over multiple agents. Such representation has several key advantages: first, our model learns a highly multimodal distribution that captures diverse future outcomes. Second, the simple predictor design requires only a single L2 loss training objective, and does not depend on trajectory anchors. Third, our model is capable of learning the joint distribution for the motion of multiple agents in a permutation-invariant manner. Furthermore, we utilize a compressed trajectory representation via PCA, which improves model performance and allows for efficient computation of the exact sample log probability. Subsequently, we propose a general constrained sampling framework that enables controlled trajectory sampling based on differentiable cost functions. This strategy enables a host of applications such as enforcing rules and physical priors, or creating tailored simulation scenarios. MotionDiffuser can be combined with existing backbone architectures to achieve top motion forecasting results. We obtain state-of-the-art results for multi-agent motion prediction on the Waymo Open Motion Dataset.

==> shortcuts.tex <==
% Copy from Occupancy Networks paper

% shortcuts for bold characters (vectors, matrices)
\newcommand{\ba}{\mathbf{a}}\newcommand{\bA}{\mathbf{A}}
\newcommand{\bb}{\mathbf{b}}\newcommand{\bB}{\mathbf{B}}
\newcommand{\bc}{\mathbf{c}}\newcommand{\bC}{\mathbf{C}}
\newcommand{\bd}{\mathbf{d}}\newcommand{\bD}{\mathbf{D}}
\newcommand{\be}{\mathbf{e}}\newcommand{\bE}{\mathbf{E}}
\newcommand{\bff}{\mathbf{f}}\newcommand{\bF}{\mathbf{F}} %\bf already taken
\newcommand{\bg}{\mathbf{g}}\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}\newcommand{\bH}{\mathbf{H}}
\newcommand{\bi}{\mathbf{i}}\newcommand{\bI}{\mathbf{I}}
\newcommand{\bj}{\mathbf{j}}\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bk}{\mathbf{k}}\newcommand{\bK}{\mathbf{K}}
\newcommand{\bl}{\mathbf{l}}\newcommand{\bL}{\mathbf{L}}
\newcommand{\bm}{\mathbf{m}}\newcommand{\bM}{\mathbf{M}}
\newcommand{\bn}{\mathbf{n}}\newcommand{\bN}{\mathbf{N}}
\newcommand{\bo}{\mathbf{o}}\newcommand{\bO}{\mathbf{O}}
\newcommand{\bp}{\mathbf{p}}\newcommand{\bP}{\mathbf{P}}
\newcommand{\bq}{\mathbf{q}}\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\br}{\mathbf{r}}\newcommand{\bR}{\mathbf{R}}
\newcommand{\bs}{\mathbf{s}}\newcommand{\bS}{\mathbf{S}}
\newcommand{\bt}{\mathbf{t}}\newcommand{\bT}{\mathbf{T}}
\newcommand{\bu}{\mathbf{u}}\newcommand{\bU}{\mathbf{U}}
\newcommand{\bv}{\mathbf{v}}\newcommand{\bV}{\mathbf{V}}
\newcommand{\bw}{\mathbf{w}}\newcommand{\bW}{\mathbf{W}}
\newcommand{\bx}{\mathbf{x}}\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bz}{\mathbf{z}}\newcommand{\bZ}{\mathbf{Z}}

% shortcuts for bold greek characters (vectors, matrices)
\newcommand{\balpha}{\boldsymbol{\alpha}}\newcommand{\bAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}\newcommand{\bBeta}{\boldsymbol{\Beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}\newcommand{\bEpsilon}{\boldsymbol{\Epsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}\newcommand{\bZeta}{\boldsymbol{\Zeta}}
\newcommand{\beeta}{\boldsymbol{\eta}}\newcommand{\bEta}{\boldsymbol{\Eta}} % \beta already taken
\newcommand{\btheta}{\boldsymbol{\theta}}\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\biota}{\boldsymbol{\iota}}\newcommand{\bIota}{\boldsymbol{\Iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}\newcommand{\bKappa}{\boldsymbol{\Kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}\newcommand{\bMu}{\boldsymbol{\Mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}\newcommand{\bNu}{\boldsymbol{\Nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bomikron}{\boldsymbol{\omikron}}\newcommand{\bOmikron}{\boldsymbol{\Omikron}}
\newcommand{\bpi}{\boldsymbol{\pi}}\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\brho}{\boldsymbol{\rho}}\newcommand{\bRho}{\boldsymbol{\Rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}\newcommand{\bTau}{\boldsymbol{\Tau}}
\newcommand{\bypsilon}{\boldsymbol{\ypsilon}}\newcommand{\bYpsilon}{\boldsymbol{\Ypsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bchi}{\boldsymbol{\chi}}\newcommand{\bChi}{\boldsymbol{\Chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}\newcommand{\bOmega}{\boldsymbol{\Omega}}

% shortcuts for blackboard bold characters (eg, number sets)
\newcommand{\nA}{\mathbb{A}}
\newcommand{\nB}{\mathbb{B}}
\newcommand{\nC}{\mathbb{C}}
\newcommand{\nD}{\mathbb{D}}
\newcommand{\nE}{\mathbb{E}}
\newcommand{\nF}{\mathbb{F}}
\newcommand{\nG}{\mathbb{G}}
\newcommand{\nH}{\mathbb{H}}
\newcommand{\nI}{\mathbb{I}}
\newcommand{\nJ}{\mathbb{J}}
\newcommand{\nK}{\mathbb{K}}
\newcommand{\nL}{\mathbb{L}}
\newcommand{\nM}{\mathbb{M}}
\newcommand{\nN}{\mathbb{N}}
\newcommand{\nO}{\mathbb{O}}
\newcommand{\nP}{\mathbb{P}}
\newcommand{\nQ}{\mathbb{Q}}
\newcommand{\nR}{\mathbb{R}}
\newcommand{\nS}{\mathbb{S}}
\newcommand{\nT}{\mathbb{T}}
\newcommand{\nU}{\mathbb{U}}
\newcommand{\nV}{\mathbb{V}}
\newcommand{\nW}{\mathbb{W}}
\newcommand{\nX}{\mathbb{X}}
\newcommand{\nY}{\mathbb{Y}}
\newcommand{\nZ}{\mathbb{Z}}

% shortcuts for calligraphic characters (sets, index sets, ...)
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% references to figures, sections, algorithms, equations, tables
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\eqnref}[1]{Eq.~\eqref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}

% argmin / argmax operators
\DeclareMathOperator*{\argmax}{argmax~}
\DeclareMathOperator*{\argmin}{argmin~}
\DeclareMathOperator{\EX}{\mathbb{E}}

% mathcal / mathbf shortcuts
\def\mc{\mathcal}
\def\mb{\mathbf}

% nice transpose operator
\newcommand{\T}{^{\raisemath{-1pt}{\mathsf{T}}}}

% statistical dependency symbol (_||_)
\newcommand{\Perp}{\perp\!\!\! \perp}

% shortcuts for: \eg, \ie, \cf, \etc, \vs, \wrt, \dof, \etal, \iid
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{cf\onedot} \def\Cf{Cf\onedot}
\def\etc{etc\onedot}
\def\vs{vs\onedot}
\def\wrt{wrt\onedot}
\def\dof{d.o.f\onedot}
\def\etal{et~al\onedot}
\def\iid{i.i.d\onedot}
\makeatother

% nice url font and color
\renewcommand\UrlFont{\color{blue}\rmfamily}

% rotation
\newcommand*\rot{\rotatebox{90}}

% boldparagraph for unnumbered sections
\newcommand{\boldparagraph}[1]{\vspace{0.1em}\noindent{\bf #1.}}

\definecolor{darkgreen}{rgb}{0,0.7,0}



\newcommand{\todo}[1]{\noindent{\color{red}{{\bf TODO:} {#1}}}}

% commands for comments
\newcommand{\red}[1]{\noindent{\color{red}{#1}}}
\newcommand{\black}[1]{#1}
\newcommand{\lightred}[1]{\noindent{\color{lightred}{#1}}}
\newcommand{\songyou}[1]{ \noindent {\color{NavyBlue} {\bf Songyou:} {#1}} }


% fft / ifft
\def\fft{\text{FFT}}
\def\ifft{\text{IFFT}}

% highlighted yes / no
\def\yes{\noindent{\color{ForestGreen}{Yes}}}
\def\no{\noindent{\color{WildStrawberry}{No}}}


% highlighted cross / tick
%\newcommand{\cmark}{\color{ForestGreen}{\ding{52}}}%
%\newcommand{\xmark}{\color{WildStrawberry}{\ding{56}}}%
\newcommand{\cmark}{\color{ForestGreen}{\ding{51}}}%
\newcommand{\xmark}{\color{WildStrawberry}{\ding{55}}}%


% horizontally and vertically center align  of table cell
\newcolumntype{P}[1]{>{\centering\arraybackslash}m{#1}}

\newcommand{\dummyfig}[1]{
  \centering
  \fbox{
    \begin{minipage}[c][0.15\textheight][c]{0.5\textwidth}
      \centering{#1}
    \end{minipage}
  }
}

==> table/latency_rebuttal.tex <==
\begin{table}[H]
% Remove space before table.
\vspace{-1em}
% \scriptsize
\small
\setlength{\tabcolsep}{1mm}
\centering
% \def\arraystretch{1.2}
\begin{tabular}{lccccccccccccc}
\specialrule{.2em}{.1em}{.1em}

Method  & \scalebox{0.9}[1.0]{Latency (ms)} & \scalebox{0.9}[1.0]{minSADE($\downarrow$)} & \scalebox{0.9}[1.0]{minSFDE($\downarrow$)} & \scalebox{0.9}[1.0]{SMissRate($\downarrow$)} \\ \hline
Ours ($T=8$)   & 101.0 & 0.91 & 2.06 & 0.47 \\ 
Ours ($T=16$)  & 203.7 & 0.88 & 1.96 & 0.44 \\
Ours ($T=32$)  & 408.5 & 0.88 & 1.97 & 0.43 \\

\specialrule{.1em}{.05em}{.05em}

\end{tabular}
% Remove space after table.
\label{table:latency_rebuttal}
\vspace{-1.2em}
\end{table}

==> table/womd_marginal.tex <==

% \begin{table}[t]
% \scriptsize
% \setlength{\tabcolsep}{1mm}
% \centering
% % \def\arraystretch{1.2}
% \begin{tabular}{lccccccccccccc}
% \specialrule{.2em}{.1em}{.1em}
% % Method & Soft mAP($\uparrow$) &  mAP($\uparrow$) & minADE($\downarrow$) & minFDE($\downarrow$) & MissRate($\downarrow$) & ADE($\downarrow$) & FDE($\downarrow$) \\ \hline
% Method & Soft mAP &  mAP & minADE & minFDE & MissRate & ADE & FDE \\
%  & ($\uparrow$) &  ($\uparrow$) & ($\downarrow$) & ($\downarrow$) & ($\downarrow$) & ($\downarrow$) & ($\downarrow$) \\ \hline
% SceneTransformer~\cite{ngiam21scene_transformer}   & - & 0.279 & 0.612 & 1.212 & 0.156 \\
% DenseTNT~\cite{gu21dense_tnt}                      & - & 0.328 & 1.039 &	1.551 &	0.157 \\
% MultiPath\cite{sapp2020multipath}                  & - & 0.409 & 0.880 & 2.040 & 0.345 \\
% MultiPath++\cite{varadarajan2021multipath++}       & - & 0.409 & 0.556 & 1.158 & 0.134 \\
% MTR-A~\cite{shi2022mtr}                            & \bf{0.459} & \bf{0.449} & 0.564 & 1.134 & 0.116  \\
% Wayformer~\cite{nayakanti2022wayformer}            & - & 0.419 & \bf{0.545} & \bf{1.128} & \bf{0.123} & 1.216 & 2.680  \\

% %MotionDiffuser (Ours, pca_temp_0.5)                              & 0.402 & 0.382 &	0.587 &	1.232 & 0.143 \\
% MotionDiffuser (Ours)                              & 0.415 & 0.394 & 0.575 &	1.210 & 0.140 & \bf{1.212} & \bf{2.678} \\

% \specialrule{.1em}{.05em}{.05em}

% \end{tabular}
% \caption{Marginal prediction on Waymo Open Motion Dataset}

% \label{table:womd_marginal}
% \end{table}

\begin{table}[t]
\scriptsize
\setlength{\tabcolsep}{1mm}
\centering
% \def\arraystretch{1.2}
\begin{tabular}{lccccccccccccc}
\specialrule{.2em}{.1em}{.1em}
% Method & Soft mAP($\uparrow$) &  mAP($\uparrow$) & minADE($\downarrow$) & minFDE($\downarrow$) & MissRate($\downarrow$) \\ \hline
Method & Soft mAP &  mAP & minADE & minFDE & MissRate \\
 & ($\uparrow$) &  ($\uparrow$) & ($\downarrow$) & ($\downarrow$) & ($\downarrow$) \\ \hline
SceneTransformer~\cite{ngiam21scene_transformer}   & - & 0.279 & 0.612 & 1.212 & 0.156 \\
DenseTNT~\cite{gu21dense_tnt}                      & - & 0.328 & 1.039 &	1.551 &	0.157 \\
MultiPath\cite{sapp2020multipath}                  & - & 0.409 & 0.880 & 2.040 & 0.345 \\
MultiPath++\cite{varadarajan2021multipath++}       & - & 0.409 & 0.556 & 1.158 & 0.134 \\
MTR-A~\cite{shi2022mtr}                            & \bf{0.459} & \bf{0.449} & 0.564 & 1.134 & 0.116 \\
Wayformer~\cite{nayakanti2022wayformer}            & - & 0.419 & \bf{0.545} & \bf{1.128} & \bf{0.123} \\
 MotionDiffuser (Ours)                              & 0.415 & 0.393 & 0.563 &	1.162 & 0.131 \\
%MotionDiffuser (Ours)                              & 0.402 & 0.382 &	0.587 &	1.232 & 0.143 \\

\specialrule{.1em}{.05em}{.05em}

\end{tabular}
\caption{Marginal prediction on Waymo Open Motion Dataset}

\label{table:womd_marginal}
\end{table}

